Topological Computational Paths: Presentation Invariance and Observable Quotients

A computational path records the steps used to establish an equality. Topologies on computational equality witnesses can depend on the chosen generators and execution schedule, even when their algebraic and homotopical meanings agree. We study continuous presentations of finite computational paths whose declared rewrites are realized by endpoint-fixed homotopies. We compare a topology retaining the full signed trace with an observable topology recording endpoints, length, and exact path realization. Continuous finite-word interpretations that are inverse up to scoped rewriting preserve trace-sensitive quotient arrows and their final composable-pair spaces. Observable quotients behave differently. Over a point with a nonempty primitive alphabet, we classify their topology: it records length parity when all named relations preserve parity, and is otherwise indiscrete. Adjoining a conservative abbreviation can therefore turn a discrete two-element quotient into an indiscrete space, even though ordinary multiplication remains continuous. A circle presentation also gives nonhomeomorphic quotients under binary and equal-slot timing. Geometric completeness alone does not identify the trace-sensitive and observable topologies. Multiplication is continuous on the quotient of composable representatives. We characterize when this topology agrees with the ordinary pullback topology and give an open-projection criterion. Universal presentations recover classical fundamental-groupoid topology. Normal forms, primitive interchange, and a Cayley covering prove completeness for circle, torus, product, and rose presentations. A literal-word correspondence relates the semantics to the reflexivity, symmetry, and transitivity fragment of equality derivations. Selected results are formalized in Lean, with the realization models and proof coverage stated explicitly.

==> figures/backtracking.tex <==
\begin{figure}[htbp]
\centering
\begin{tikzpicture}[font=\small,>=Stealth,x=4.7cm,y=2.8cm]
\draw[->] (0,0) -- (1.12,0) node[right] {$t$};
\draw[->] (0,0) -- (0,1.18) node[above] {parameter of $\alpha$};
\draw[pathblue,very thick] (0,0) -- (0.5,1) -- (1,0);
\draw[pathorange,thick,dashed] (0,0) -- (0.25,0.5) -- (0.75,0.5) -- (1,0);
\draw[pathteal,thick,dash dot] (0,0) -- (0.125,0.25) -- (0.875,0.25) -- (1,0);
\draw[black,very thick] (0,0) -- (1,0);
\node[below left] at (0,0) {$0$};
\node[below] at (0.5,0) {$\tfrac12$};
\node[below] at (1,0) {$1$};
\node[left] at (0,1) {$1$};
\node[pathblue,anchor=west] at (1.22,0.95) {$u=0$: full out-and-back};
\node[pathorange,anchor=west] at (1.22,0.65) {$u=\tfrac12$: turn halfway};
\node[pathteal,anchor=west] at (1.22,0.35) {$u=\tfrac34$: turn at one quarter};
\node[anchor=west] at (1.22,0.05) {$u=1$: constant at $\alpha(0)$};
\end{tikzpicture}
\caption{Backtracking cancellation as an explicit homotopy.
The plotted function is $r_u(t)=\min\{2t,2(1-t),1-u\}$;
the actual path is $H(u,t)=\alpha(r_u(t))$.
As $u$ increases, the turning point retreats along $\alpha$ and the path
waits there before returning.  All intermediate paths stay in $\alpha(I)$,
so even a hole surrounded by $\alpha$ cannot obstruct this cancellation.}
\label{fig:backtracking}
\end{figure}



==> figures/coherence.tex <==
\begin{figure}[htbp]
\centering
\begin{tikzpicture}[font=\small,>=Stealth,scale=1.12]
\foreach \x/\lab in {0/{(a) In the plane},4.6/{(b) In the punctured plane}} {
 \begin{scope}[xshift=\x cm]
 \node[font=\small\bfseries] at (1.6,2.75) {\lab};
 \fill[pathteal!7] (0,0) -- (1.6,1.8) -- (3.2,0) -- cycle;
 \draw[->,pathblue,thick] (0,0) -- (1.6,1.8);
 \draw[->,pathblue,thick] (1.6,1.8) -- (3.2,0);
 \draw[->,pathorange,thick] (0,0) -- (3.2,0);
 \fill (0,0) circle(1.5pt) node[below left] {$A$};
 \fill (1.6,1.8) circle(1.5pt) node[above] {$B$};
 \fill (3.2,0) circle(1.5pt) node[below right] {$C$};
 \node[pathblue] at (0.55,1.1) {$\alpha$};
 \node[pathorange] at (1.6,-0.28) {$\beta$};
 \end{scope}
}
\foreach \h in {0.45,0.9,1.35} {
 \draw[pathteal,dashed] (0,0) -- (1.6,\h) -- (3.2,0);
}
\draw[->,pathteal] (1.6,1.6) -- (1.6,0.2);
\draw[fill=white,thick] (6.2,0.6) circle(0.085);
\node[anchor=south,inner sep=1pt] at (6.2,0.77) {$O\notin X$};
\node[align=center] at (1.6,-0.95) {$H(u,t)=(1-u)\alpha(t)+u\beta(t)$\\
 $\alpha\simeq_{\partial I}\beta$};
\node[align=center] at (6.2,-0.95) {$\left|\operatorname{wind}_{O}
 (\alpha\star\beta^{-1})\right|=1$\\
 $\alpha\not\simeq_{\partial I}\beta$};
\end{tikzpicture}
\caption{Coherence requires a homotopy inside the chosen ambient space.
Left: intermediate broken paths move $B$ to the segment $AC$, keeping $A,C$
fixed.  Right: deleting the interior point $O=(0,\tfrac13)$ prevents any
such homotopy, although both boundary paths remain continuous.
For $|p|=\alpha$, $(p,\beta)$ is coherent only in the left-hand example.
The shaded triangle is available in (a), but is not a filling in (b).}
\label{fig:coherence}
\end{figure}



==> figures/normal-form.tex <==
\begin{figure}[htbp]
\centering
\begin{tikzpicture}[font=\small,>=Stealth]
\node (geo) at (0,2) {$h(u)=h(v)$};
\node (code) at (0,0.9) {$N(u)=N(v)$};
\draw[->,pathteal,thick] (geo) -- (code)
 node[midway,right] {\quad(b) semantic separation};
\node (common) at (0,-0.25) {$\nu(N(u))=\nu(N(v))$};
\draw[->] (code) -- (common) node[midway,right] {\quad apply $\nu$};
\node (u) at (-3.8,-0.25) {$u$};
\node (v) at (3.8,-0.25) {$v$};
\draw[pathblue,thick] (u) -- (common)
 node[midway,above] {$\approx$} node[midway,below] {(a)};
\draw[pathblue,thick] (common) -- (v)
 node[midway,above] {$\approx$} node[midway,below] {(a), symmetry};
\end{tikzpicture}
\caption{A normal-form certificate proves completeness by two different
means: syntactic normalization (a) connects each trace to its chosen normal
representative; semantic separation (b) forces the two codes to agree.
The bottom row is then scoped transitivity, yielding $u\approx v$.
The arrows are logical steps and assume nothing about continuity of $N$ or
$\nu$.}
\label{fig:normal-form}
\end{figure}


==> figures/oriented-steps.tex <==
\begin{figure}[!htbp]
\centering
\begin{tikzpicture}[font=\small,>=Stealth]
\node[anchor=west,font=\small\bfseries] at (-0.2,2.6) {(a) Labelled computation};
\node (a) at (0,1.55) {$a$};
\node (b) at (2,1.55) {$b$};
\node (c) at (4,1.55) {$c$};
\draw[->,pathblue,thick] (a) -- node[above] {$r$} (b);
\draw[->,pathblue,thick] (b) -- node[above] {$s$} (c);
\draw[->,pathblue] (a) to[bend left=20] node[above] {$p=r;s$} (c);
\draw[->,pathorange] (a) to[bend right=28] node[below] {$u$} (c);
\node[align=center] at (2,0.25) {Parallel witnesses from $a$ to $c$};
\node[anchor=west,font=\small\bfseries] at (5.25,2.6) {(b) Rewriting and realization};
\node[draw=pathblue,rounded corners,fill=pathblue!5,align=center,
  inner sep=5pt] (rewrite) at (7.9,1.95)
  {$p\RwEq u$\\when the scoped rules derive it};
\node (homotopy) at (7.9,0.45) {$|p|\simeq_{\partial I}|u|$};
\draw[->,pathteal,thick] (rewrite) -- node[right] {soundness} (homotopy);
\draw[gray!50] (-0.2,-0.15) -- (10.6,-0.15);
\node[align=center,font=\footnotesize] at (5.2,-0.65)
 {Formal reversal: $e^+\in E^+\cong E$, $e^-\in E^-\cong E$\\[2pt]
 $\widetilde s(e^-)=t(e),\quad \widetilde t(e^-)=s(e),\qquad
 \widetilde\rho(e^-)(t)=\rho(e)(1-t)$};
\end{tikzpicture}
\caption{Labels record a route and its composition. A scoped rewrite between
parallel witnesses gives an endpoint-fixed homotopy of their realizations by
soundness; the converse requires geometric completeness. Formal reversal
traverses a represented path in the opposite direction and leaves the topology
of the step space unchanged. Endpoint maps take values in $X$; the realization
map takes values in $X^I$.}
\label{fig:oriented-steps}
\end{figure}



==> figures/universal-section.tex <==
\begin{figure}[htbp]
\centering
\begin{tikzcd}[column sep=5em,row sep=4em,
 every label/.append style={font=\normalsize},
 every cell/.append style={font=\large}]
 X^I \arrow[r,shift left=1ex,"\sigma"] \arrow[d,"q_I"']
 & T_{\mathcal U_X}^{*} \arrow[l,shift left=1ex,"\pi"] \arrow[d,"q_*"] \\
 \Pi_1^q(X) \arrow[r,shift left=1ex,"\overline\sigma"]
 & G_{\mathcal U_X}^{*} \arrow[l,shift left=1ex,"\overline\pi"]
\end{tikzcd}

\smallskip
\(\displaystyle
 \pi\sigma=\mathrm{id}_{X^I},\qquad
 G_{\mathcal U_X}^{\mathrm{tr}}\cong\Pi_1^q(X)
 \cong G_{\mathcal U_X}^{\mathrm{obs}}.
\)
\caption{The universal one-letter section supplies the topology, and the
universal rules supply the equivalence relation.  Here
$*\in\{\mathrm{tr},\mathrm{obs}\}$ and
$\sigma(\gamma)=(\langle\gamma\rangle,\gamma)$; $q_I$ is the homotopy
quotient map.  The lower maps are induced by $\sigma$ and $\pi$.
The upper maps are continuous, with $\pi\sigma=\mathrm{id}$, so $\pi$ is
quotient.  Agreement of scoped and homotopy relations makes the lower maps
mutually inverse homeomorphisms.  Under these identifications, $J_{\mathcal U_X}$
is the identity on path classes.}
\label{fig:universal-section}
\end{figure}



==> figures/winding.tex <==
\begin{figure}[htbp]
\centering
\begin{tikzpicture}[font=\small,>=Stealth]
\node[font=\small\bfseries] at (1.7,3.9) {(a) Circle: lift endpoint $2$};
\draw[->] (0,0) -- (3.5,0) node[right] {$t$};
\draw[->] (0,0) -- (0,2.9) node[above] {$\widetilde\gamma(t)$};
\draw[pathblue,thick] (0,0) .. controls (0.55,1.6) and (1.15,0.25) .. (1.65,1.4)
 .. controls (2.25,2.8) and (2.7,1.65) .. (3.15,2.4);
\draw[pathorange,thick,dashed] (0,0) -- (3.15,2.4);
\fill (3.15,2.4) circle (1.6pt);
\node[left] at (0,2.4) {$2$};
\node[below] at (3.15,0) {$1$};
\node[pathorange,rotate=35] at (1.55,0.77) {$t\mapsto 2t$};
\node[font=\small\bfseries] at (6.75,3.9) {(b) Torus: lift endpoint $(2,1)$};
\begin{scope}[xshift=5.1cm,x=1.5cm,y=2.4cm]
\draw[step=1,gray!25,very thin] (0,0) grid (2,1);
\draw[->] (-0.1,0) -- (2.25,0);
\draw[->] (0,-0.08) -- (0,1.15);
\draw[pathblue,very thick,->] (0,0) -- (2,0);
\draw[pathblue,very thick,->] (2,0) -- (2,1);
\draw[pathorange,thick,dashed,->] (0,0) -- (2,1);
\fill (0,0) circle(1.1pt) node[below left] {$(0,0)$};
\fill (2,1) circle(1.1pt) node[above right] {$(2,1)$};
\node[pathblue,below] at (1,0) {$a^2$};
\node[pathblue,right] at (2,0.5) {$b$};
\node[pathorange,rotate=37] at (0.8,0.58) {$(2t,t)$};
\end{scope}
\end{tikzpicture}
\caption{Winding separates normal forms because lifts remember endpoints.
Left: a lift beginning at $0$ and ending at $2$ is straightened to $2t$.
Right: the sequential word $a^2;b$ and the simultaneous loop have lifts
with common endpoints $(0,0)$ and $(2,1)$; straight-line interpolation in
$\mathbb R^2$ gives a homotopy after projection to the torus.
Both plots are drawn in the covering spaces $\mathbb R$ and $\mathbb R^2$.}
\label{fig:winding}
\end{figure}


